Measurement of the $ZZ$ production cross section in $pp$ collisions at $\sqrt{s}$ = 8 TeV using the $ZZ\to\ell^{-}\ell^{+}\ell^{\prime -}\ell^{\prime +}$ and $ZZ\to\ell^{-}\ell^{+}\nu\bar{\nu}$ channels with the ATLAS detector

A measurement of the $ZZ$ production in the $\ell^{-}\ell^{+}\ell^{\prime -}\ell^{\prime +}$ and $\ell^{-}\ell^{+}\nu\bar{\nu}$ channels $(\ell = e, \mu)$ in proton--proton collisions at $\sqrt{s} = 8$ TeV at the Large Hadron Collider at CERN, using data corresponding to an integrated luminosity of 20.3 fb$^{-1}$ collected by the ATLAS experiment in 2012 is presented. The fiducial cross sections for $ZZ\to\ell^{-}\ell^{+}\ell^{\prime -}\ell^{\prime +}$ and $ZZ\to \ell^{-}\ell^{+}\nu\bar{\nu}$ are measured in selected phase-space regions. The total cross section for $ZZ$ events produced with both $Z$ bosons in the mass range 66 to 116 GeV is measured from the combination of the two channels to be $7.3\pm0.4\textrm{(stat)}\pm0.3\textrm{(syst)}\pm0.2\textrm{(lumi)}$ pb, which is consistent with the Standard Model prediction of $6.6^{+0.7}_{-0.6}$ pb. The differential cross sections in bins of various kinematic variables are presented. The differential event yield as a function of the transverse momentum of the leading $Z$ boson is used to set limits on anomalous neutral triple gauge boson couplings in $ZZ$ production.

==> acknowledgements/Makefile <==
# Makefile for creating ATLAS Acknowledegments

TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf

BASENAME = Acknowledgements-main

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $$file"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *~

cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf

